What is the Effect of Importance Weighting in Deep Learning?

Importance-weighted risk minimization is a key ingredient in many machine learning algorithms for causal inference, domain adaptation, class imbalance, and off-policy reinforcement learning. While the effect of importance weighting is well-characterized for low-capacity misspecified models, little is known about how it impacts over-parameterized, deep neural networks. This work is inspired by recent theoretical results showing that on (linearly) separable data, deep linear networks optimized by SGD learn weight-agnostic solutions, prompting us to ask, for realistic deep networks, for which many practical datasets are separable, what is the effect of importance weighting? We present the surprising finding that while importance weighting impacts models early in training, its effect diminishes over successive epochs. Moreover, while L2 regularization and batch normalization (but not dropout), restore some of the impact of importance weighting, they express the effect via (seemingly) the wrong abstraction: why should practitioners tweak the L2 regularization, and by how much, to produce the correct weighting effect? Our experiments confirm these findings across a range of architectures and datasets.

==> sections/related.tex <==
%
% Paragraph on the Importance of Importance weighting
%
Importance sampling allows one to estimate some properties of a \emph{target} distribution $q$, 
when only a \emph{source} distribution $p$, is available to be sampled from.
\citep{horvitz1952generalization, kahn1953methods, rubinstein2016simulation, koller2009probabilistic}.
Concretely, given $n$ samples $x_1, ..., x_n \sim p(x)$,
and the task of estimating some function of the data, 
say $f(x)$, under the target distribution $E_q[f(x)]$,
importance sampling produces an unbiased estimate 
%for the desired quantity 
by weighting each sample $x$ 
according to the likelihood ratio $q(x)/p(x)$:
% \begin{equation*}
\begin{align*}
\mathbbm{E}_p\left[ \frac{q(x)}{p(x)} f(x)\right]
&= \int_{x} f(x) \frac{q(x)}{p(x)} p(x) dx \\
= \int_{x} f(x) q(x) dx &= \mathbbm{E}_q\left[f(x)\right]
\end{align*}
% \end{equation*}
Machine learning practitioners commonly exploit 
this idea in two ways:
(i) by re-sampling to correct for the discrepancy in likelihood 
or (ii) by weighting examples according to the likelihood ratio \citep{rubinstein2016simulation, shimodaira2000improving, koller2009probabilistic}. 
The latter approach underlies the common method of \emph{importance-weighted empirical risk minimization (IW-ERM)}.

When the likelihood ratio is known, 
importance sampling offers unbiased estimates
of the generalization error \citep{Cortes2008sample}, 
and IW-ERM optimizes an unbiased estimate 
of the loss function on distribution $q$.
However, this unbiasedness can come at the cost of significant variance---when for some values of $x$, $q(x)>>p(x)$, importance weights can grow arbitrarily large. 
% While a great body of research addresses 
% this bias-variance trade-off \citep{neal2001annealed, Cortes2008sample},
% this paper focuses on a different question: what, if anything, is the effect of IW-ERM
% when applied to a specific class of models (deep neural networks).
% % Do we need to mention bias-variance trade-off of IW when we don't discuss it again at all?


Algorithms employing IW-ERM pop up in many areas of machine learning.
Typically, in causal inference we possess only offline data, 
but wish to answer counterfactual questions,
estimating the statistical properties 
that might hold \emph{were we to intervene},
mutating the probability distribution \citep{rosenbaum1983central}.
% that might hold were to intervene mutating the probability distribution that generates our data \cite{rosenbaum1983central}.
More recently, \cite{johansson2018learning} 
employ weighted risk minimization in a study aimed at estimating causal effects using deep neural networks. 

In off-policy reinforcement learning,
we wish to evaluate a target policy $\pi_t$, 
using only trajectories sampled from a source $\pi_s$.
In the bandit literature, where importance sampling is sometimes known by the alias \emph{inverse propensity scoring} \citep{horvitz1952generalization, dudik2011doubly, agarwal2014taming},
the technique is especially important,
because it can be prohibitively expensive to collect a fresh set of data (by interacting with the environment)
every time we wish to evaluate a proposed policy.
Importance sampling is also found in the literature on temporal difference learning in Markov decision processes \citep{precup2000eligibility, precup2001off}.
More recently, various applications of importance sampling have emerged in the modern literature on learning from logged contextual bandit feedback with deep networks \citep{joachims2018deep},
deep reinforcement learning \citep{pinto2016supersizing}, 
and deep imitation learning \citep{murali2016tsc}. 
Another deep reinforcement learning paper uses weighted sampling to choose experiences from the replay buffer for performing TD updates \citep{schaul2015prioritized}. 
However, these weights are not based on likelihood ratios, but instead are heuristically chosen 
to be proportional to the Bellman errors for those experiences.

Weighted ERM is also used in active learning, where one hopes to correct for deliberate sample selection bias \citep{Beygelzimer2009importance}, and in domain adaptation, to learn a classifier on data sampled from the source distribution $p$ that minimizes error on a target distribution $q$.
While domain adaptation is impossible in general, under the covariate shift (sample selection bias) assumption \citep{shimodaira2000improving}
or label shift (also called prior probability shift) \citep{elkan2001foundations}, 
models can be improved by incorporating unlabeled target data, often through IW-ERM. 
Recently, \citet{lipton2018detecting}
introduced a consistent estimator for the test set label distribution under mild conditions, 
demonstrating that deep neural networks 
can be improved through retraining with accurately estimated importance weights.
% Our experiments also address the label shift scenario.

% Recently, \citet{soudry2017implicit} investigated the open question of why neural networks generalize.
Recently, \citet{soudry2017implicit} investigated explanations for the generalization abilities of neural networks.
Problematically, given a fixed neural network architecture, there exist infinitely many sets of parameters that achieve empirical risk arbitrarily close to $0$, most of which generalize poorly to unseen data. 
Thus determining precisely why neural networks generalize requires understanding the behavior of the optimization algorithm, typically a variant of stochastic gradient descent (SGD). 
When optimizing square loss and initialized at the origin, 
SGD is known to converge to the minimum Euclidean norm solution.
However, when optimizing cross-entropy loss on a classification task,
there is no finite optimal solution when the data is separable.
This is easy to see in the linear case (logistic regression),
where the loss can always be driven further down by scaling up the weights, $\lim_{t \rightarrow \infty} \ell(y,\sigma(w_t x)) = 0 \Rightarrow \lim_{t\rightarrow \infty} ||w_t|| =  \infty$.
Here $\ell$ is the loss, $\sigma$ is the sigmoid activation function, and $w_t$ 
is the value of the weights at iteration $t$ of SGD.
If only the direction of the weights 
but not their magnitude,
determines the partitioning of the data into classes, then what does the \emph{direction} of $w_t/||w_t||$ converge to? \citet{soudry2017implicit} show that for linear models
it converges to the solution 
of the hard-margin \emph{support vector machine (SVM)}.
These results hold on linear networks with no hidden layers
and were subsequently extended 
to deep fully-connected linear networks 
in \citet{gunasekar2018implicit}, 
which also analyzes linear convolutional networks, 
showing that for these nets, the solution is
related to the bridge penalty in the frequency domain.


% risk minimization,
% in which we unequally weight the contribution 
% of each data point to our objective 
% appears throughout machine learning and statistics.
% In domain adaptation, we can often produce better models 
% target data by training on the source data with carefully chosen weights \citep{shimodaira2000improving}. 
% In active learning, importance weighting is commonly used 
% to to correct for the sampling bias \citep{Beygelzimer2009importance}.
% The technique is widely used in off-policy reinforcement learning,
% where we hope, by re-weighting stale experiences,
% to evaluate a policy

%
% Connect to causality
%
% Importance weighting is deeply connected to causality
% because we are 

% --- propensity scoring \cite{rosenbaum1983central}
% learning from logged bandit feedback \cite{swaminathan2015counterfactual}
%
% Recent developments in theory of deep learning / stochastic gradient descent.   
%



% \newpage

% Faced with domain adaptation, 
% we often fit predictors by weighting each example 
% by the density ratio $q(x,y)/p(x,y)$
% where $q$ denotes the target distribution. 
% and $p$ denotes the source distribution.
% This technique underlies much work on co-variate shift,
% and is known to be especially important 
% in the setting of model misspecification \cite{shimodaira2000improving}.






%
%  Questions raised about 
%       a) does importance weighting do anything at all?
%       b) interplay between importance weighting and early stopping
%       c) 
%




% Importance weighting is a widely used technique, in machine learning (distribution shift, unbalanced datasets, monte carlo methods, off-policy learning, active learning, causal models). Lipton et al. \cite{} show that re-weighting of training examples to correct for label shift at test-time improves test accuracy, and  However, there is a lack of detailed empirical exploration of the effects of this technique for deep networks. We are motivated by recent work from Nacson et al \cite{} which shows that logistic regression trained with SGD on linearly separable data converges in direction to the $L_2$ max margin separator, noting similar observed behavior in deep networks. This raises the question of how to reconcile the wide use of importance weighting with this recent theoretical result. 

% We seek to answer the following questions:
% \begin{itemize}
% \item Do deep networks converge to solutions independently of importance weighting?
% \item What effect is importance weighting having on these models?
% \item Do deep networks
% \end{itemize}




% \paragraph{Deep learning optimization}
% \begin{itemize}
%     \item \cite{soudry2017implicit}
%     \item \cite{gunasekar2018implicit}
%     \item ...
% \end{itemize}


% \paragraph{Classic importance weighting}
% \begin{itemize}
%     \item Covariate shift guys \cite{shimodaira2000improving}
%     \item \cite{sugiyama2007covariate}
%     \item ACTIVE LEARNING
%     \item \cite{Beygelzimer2009importance}
%     \item Fredrik Johansson---Generalization across designs \cite{johansson2018learning}
% \end{itemize}

% \paragraph{Papers relying on importance weighting + deep learning}

% \begin{itemize}
%     \item Prioritized experience replay \cite{schaul2015prioritized}
%     \item Label shift \citep{lipton2018detecting}
%     \item .
%     \item .
%     \item . [FIND SOME COUNTERFACUTAL STUFF and OFF-POLICY RL STUFF]
%     \item ... IW-autoencoders \cite{burda2015importance}
% \end{itemize}
